RelExt: Relation Extraction using Deep Learning approaches for Cybersecurity Knowledge Graph Improvement

Security Analysts that work in a `Security Operations Center' (SoC) play a major role in ensuring the security of the organization. The amount of background knowledge they have about the evolving and new attacks makes a significant difference in their ability to detect attacks. Open source threat intelligence sources, like text descriptions about cyber-attacks, can be stored in a structured fashion in a cybersecurity knowledge graph. A cybersecurity knowledge graph can be paramount in aiding a security analyst to detect cyber threats because it stores a vast range of cyber threat information in the form of semantic triples which can be queried. A semantic triple contains two cybersecurity entities with a relationship between them. In this work, we propose a system to create semantic triples over cybersecurity text, using deep learning approaches to extract possible relationships. We use the set of semantic triples generated through our system to assert in a cybersecurity knowledge graph. Security Analysts can retrieve this data from the knowledge graph, and use this information to form a decision about a cyber-attack.

==> relwork.tex <==

% \cite
% Abstract
% ---------

\cite{qi2014systems}
Systems and methods are disclosed to perform relation extraction in text by applying a convolution strategy to determine a kernel between sentences; applying one or more semi-supervised strategies to the kernel to encode syntactic and semantic information to recover a relational pattern of interest; and applying a classifier to the kernel to identify the relational pattern of interest in the text in response to a query.

---------------------------------------------------------------


\cite{gruber1993}
To support the sharing and reuse of formally represented knowledge among AI systems, it is useful to define the common vocabulary in which shared knowledge is represented. A specification of a representational vocabulary for a shared domain of discourse—definitions of classes, relations, functions, and other objects—is called an ontology. This paper describes a mechanism for defining ontologies that are portable over representation systems. Definitions written in a standard format for predicate calculus are translated by a system called Ontolingua into specialized representations, including frame-based systems as well as relational languages. This allows researchers to share and reuse ontologies, while retaining the computational benefits of specialized implementations.

We discuss how the translation approach to portability addresses several technical problems. One problem is how to accommodate the stylistic and organizational differences among representations while preserving declarative content. Another is how to translate from a very expressive language into restricted languages, remaining system-independent while preserving the computational efficiency of implemented systems. We describe how these problems are addressed by basing Ontolingua itself on an ontology of domain-independent, representational idioms.
---------------------------------------------------------------

\cite{undercofferIDS}

We have produced an ontology specifying a model of
computer attack. Our ontology is based upon an analysis of
over 4,000 classes of computer intrusions and their corresponding attack strategies and is categorized according to:
system component targeted, means of attack, consequence of
attack and location of attacker. We argue that any taxonomic
characteristics used to define a computer attack be limited in
scope to those features that are observable and measurable
at the target of the attack. We present our model as a
target-centric ontology that is to be refined and expanded
over time. We state the benefits of forgoing dependence upon
taxonomies, in favor of ontologies, for the classification
of computer attacks and intrusions. We have specified our
ontology using the DARPA Agent Markup Language and
have prototyped it using DAMLJessKB. We present our
model as a target-centric ontology and illustrate the benefits
of utilizing an ontology lieu of a taxonomy, by presenting
a use case scenario of a distributed intrusion detection system.
---------------------------------------------------------------
\cite{jessKB}
This report describes Jess, an expert system shell and scripting language written entirely in Sun Microsystem's Java language. Jess supports the development of rule-based expert systems which can be tightly coupled to code written in the powerful, portable Java language. The syntax of the Jess language is discussed, and a comprehensive list of supported functions is presented. Guides to calling Java functions from Jess, to extending Jess by writing Java code, and to embedding Jess in Java applications are also included.
Note: this version of Jess is now in maintenence mode, and no new features will be added. Active Jess development is being done on the 6.0 versions. This manual is largely unchanged from the Jess 5.1 relase, and therefore while it accurately describes Jess 5.2, it does not properly represent the capabilities of any newer versions of Jess.
---------------------------------------------------------------
\cite{raskin}
The paper introduces and advocates an ontological semantic
approach to information security. Both the approach and its
resources, the ontology and lexicons, arc borrowed from the
field of natural language processing and adjusted to the needs
of the new domain The approach pursues the ultimate dual
goals of inclusion of natural language data sources as an
integral part of the overall data sources in information security
applications, and formal specification of the information
security community know-how for the support of routine and
time-efficient measures to prevent and counteract computer
attacks. As the first order of the day, the approach is seen by
the information security community as a powerful means to
organize and unify thc terminology and nomenclature of the
field.
---------------------------------------------------------------
\cite{pawarRelSurvey}
With the advent of the Internet, large amount of digital text is generated everyday in the form of news articles, research publications, blogs, question answering forums and social media. It is important to develop techniques for extracting information automatically from these documents, as lot of important information is hidden within them. This extracted information can be used to improve access and management of knowledge hidden in large text corpora. Several applications such as Question Answering, Information Retrieval would benefit from this information. Entities like persons and organizations, form the most basic unit of the information. Occurrences of entities in a sentence are often linked through well-defined relations; e.g., occurrences of person and organization in a sentence may be linked through relations such as employed at. The task of Relation Extraction (RE) is to identify such relations automatically. In this paper, we survey several important supervised, semi-supervised and unsupervised RE techniques. We also cover the paradigms of Open Information Extraction (OIE) and Distant Supervision. Finally, we describe some of the recent trends in the RE techniques and possible future research directions. This survey would be useful for three kinds of readers - i) Newcomers in the field who want to quickly learn about RE; ii) Researchers who want to know how the various RE techniques evolved over time and what are possible future research directions and iii) Practitioners who just need to know which RE technique works best in various settings.
---------------------------------------------------------------
\cite{bachRelSurvey}
Many applications in information extraction, natural language understanding, information retrieval require an understanding of the semantic relations between
entities. We present a comprehensive review of various aspects of the entity relation extraction task. Some of the most important supervised and semi-supervised
classification approaches to the relation extraction task are covered in sufficient
detail along with critical analyses. We also discuss extensions to higher-order relations. Evaluation methodologies for both supervised and semi-supervised methods are described along with pointers to the commonly used performance evaluation datasets. Finally, we also give short descriptions of two important applications
of relation extraction, namely question answering and biotext mining.
---------------------------------------------------------------
\cite{kambhatla}
Extracting semantic relationships between entities
is challenging because of a paucity of annotated
data and the errors induced by entity detection modules. We employ Maximum Entropy models to
combine diverse lexical, syntactic and semantic features derived from the text. Our system obtained
competitive results in the Automatic Content Extraction (ACE) evaluation. Here we present our general approach and describe our ACE results.
---------------------------------------------------------------
\cite{zhao}
Entity relation detection is a form of information extraction that finds predefined
relations between pairs of entities in text.
This paper describes a relation detection
approach that combines clues from different levels of syntactic processing using
kernel methods. Information from three
different levels of processing is considered: tokenization, sentence parsing and
deep dependency analysis. Each source of
information is represented by kernel functions. Then composite kernels are developed to integrate and extend individual
kernels so that processing errors occurring
at one level can be overcome by information from other levels. We present an
evaluation of these methods on the 2004
ACE relation detection task, using Support Vector Machines, and show that each
level of syntactic processing contributes
useful information for this task. When
evaluated on the official test data, our approach produced very competitive ACE
value scores. We also compare the SVM
with KNN on different kernels. 
---------------------------------------------------------------
\cite{yankaiKGC}
Knowledge graph completion aims to perform link prediction between entities. In this paper, we consider the
approach of knowledge graph embeddings. Recently,
models such as TransE and TransH build entity and relation embeddings by regarding a relation as translation from head entity to tail entity. We note that these
models simply put both entities and relations within
the same semantic space. In fact, an entity may have
multiple aspects and various relations may focus on
different aspects of entities, which makes a common
space insufficient for modeling. In this paper, we propose TransR to build entity and relation embeddings in
separate entity space and relation spaces. Afterwards,
we learn embeddings by first projecting entities from
entity space to corresponding relation space and then
building translations between projected entities. In experiments, we evaluate our models on three tasks including link prediction, triple classification and relational fact extraction. Experimental results show significant and consistent improvements compared to stateof-the-art baselines including TransE and TransH. The
source code of this paper can be obtained from https:
//github.com/mrlyk423/relation extraction
---------------------------------------------------------------
\cite{brin_dipre}
The World Wide Web is a vast resource for information.
At the same time it is extremely distributed. A particular type of data
such as restaurant lists may be scattered across thousands of independent
information sources in many dierent formats. In this paper, we consider
the problem of extracting a relation for such a data type from all of these
sources automatically. We present a technique which exploits the duality
between sets of patterns and relations to grow the target relation starting
from a small sample. To test our technique we use it to extract a relation
of (author,title) pairs from the World Wide Web.
---------------------------------------------------------------
\cite{snowball_2000}
Text documents often contain valuable structured data that
is hidden in regular English sentences. This data is best exploited if available as a relational table that we could use for
answering precise queries or for running data mining tasks.
We explore a technique for extracting such tables from document collections that requires only a handful of training examples from users. These examples are used to generate
extraction patterns, that in turn result in new tuples being
extracted from the document collection. We build on this
idea and present our Snowball system. Snowball introduces
novel strategies for generating patterns and extracting tuples
from plain-text documents. At each iteration of the extraction process, Snowball evaluates the quality of these patterns
and tuples without human intervention, and keeps only the
most reliable ones for the next iteration. In this paper we
also develop a scalable evaluation methodology and metrics
for our task, and present a thorough experimental evaluation
of Snowball and comparable techniques over a collection of
more than 300,000 newspaper documents.
---------------------------------------------------------------
\cite{hasegawa_clustering}

Discovering the significant relations embedded in
documents would be very useful not only for information retrieval but also for question answering and
summarization. Prior methods for relation discovery, however, needed large annotated corpora which
cost a great deal of time and effort. We propose
an unsupervised method for relation discovery from
large corpora. The key idea is clustering pairs of
named entities according to the similarity of context words intervening between the named entities.
Our experiments using one year of newspapers reveals not only that the relations among named entities could be detected with high recall and precision,
but also that appropriate labels could be automatically provided for the relations
---------------------------------------------------------------
\cite{feldman_nonclustering}
Most information extraction systems either use hand written extraction patterns
or use a machine learning algorithm that
is trained on a manually annotated corpus. Both of these approaches require
massive human effort and hence prevent
information extraction from becoming
more widely applicable. In this paper we
present URES (Unsupervised Relation
Extraction System), which extracts relations from the Web in a totally unsupervised way. It takes as input the
descriptions of the target relations, which
include the names of the predicates, the
types of their attributes, and several seed
instances of the relations. Then the system downloads from the Web a large collection of pages that are likely to contain
instances of the target relations. From
those pages, utilizing the known seed instances, the system learns the relation
patterns, which are then used for extraction. We present several experiments in
which we learn patterns and extract instances of a set of several common IE relations, comparing several pattern
learning and filtering setups. We demonstrate that using simple noun phrase tagger is sufficient as a base for accurate
patterns. However, having a named entity recognizer, which is able to recognize the types of the relation attributes
significantly, enhances the extraction
performance. We also compare our approach with KnowItAll’s fixed generic
patterns.
---------------------------------------------------------------
\cite{cyber_trends_oxford}
Technology is rapidly evolving in a world driven by social networks, online transactions, cloud computing, and automated processes. But with the technological evolution comes the progress of cybercrime, which continually develops new attack types, tools and techniques that allow attackers to penetrate more complex or well-controlled environments, and produce increased damage and even remain untraceable. The present article aims to get an overview of the cyber-crime as it is defined and revealed by specialized literature, international legislation and historical facts, and perform an analysis of attacks reported all around the world over the last three years in order to determine patterns and trends in cyber-crime. Based on the results of the analysis, the article presents countermeasures that companies may undertake in order to ensure improved security that would support in defending their business from attackers from an information security perspective.
---------------------------------------------------------------
\cite{cyber_threat_survey}
The exponential growth of the Internet interconnections has led to a significant growth of cyber attack incidents often with disastrous and grievous consequences. Malware is the primary choice of weapon to carry out malicious intents in the cyberspace, either by exploitation into existing vulnerabilities or utilization of unique characteristics of emerging technologies. The development of more innovative and effective malware defense mechanisms has been regarded as an urgent requirement in the cybersecurity community. To assist in achieving this goal, we first present an overview of the most exploited vulnerabilities in existing hardware, software, and network layers. This is followed by critiques of existing state-of-the-art mitigation techniques as why they do or don't work. We then discuss new attack patterns in emerging technologies such as social media, cloud computing, smartphone technology, and critical infrastructure. Finally, we describe our speculative observations on future research directions.
---------------------------------------------------------------
\cite{unified_cyber_ontology}
In this paper we describe the Unified Cybersecurity Ontology (UCO) that is intended to support information integration and cyber situational awareness in cybersecurity systems. The ontology incorporates and integrates heterogeneous data and knowledge schemas from different cybersecurity systems and most commonly used cybersecurity standards for information sharing and exchange. The UCO ontology has also been mapped to a number of existing cybersecurity ontologies as well as concepts in the Linked Open Data cloud. Similar to DBpedia which serves as the core for general knowledge in Linked Open Data cloud, we envision UCO to serve as the core for cybersecurity domain, which would evolve and grow with the passage of time with additional cybersecurity data sets as they become available. We also present a prototype system and concrete use cases supported by the UCO ontology. To the best of our knowledge, this is the first cybersecurity ontology that has been mapped to general world ontologies to support broader and diverse security use cases. We compare the resulting ontology with previous efforts, discuss its strengths and limitations, and describe potential future work directions.
---------------------------------------------------------------
\cite{adap_sparse_mat}
We model knowledge graphs for their completion by encoding each entity and relation into a numerical space. All previous work including Trans(E, H, R, and D) ignore the heterogeneity (some relations link many entity pairs and others do not) and the imbalance (the number of head entities and that of tail entities in a relation could be different) of knowledge graphs. In this paper, we propose a novel approach TranSparse to deal with the two issues. In TranSparse, transfer matrices are replaced by adaptive sparse matrices, whose sparse degrees are determined by the number of entities (or entity pairs) linked by relations. In experiments, we design structured and unstructured sparse patterns for transfer matrices and analyze their advantages and disadvantages. We evaluate our approach on triplet classification and link prediction tasks. Experimental results show that TranSparse outperforms Trans(E, H, R, and D) significantly, and achieves state-of-the-art performance.
---------------------------------------------------------------
\cite{transe_bordes}
We consider the problem of embedding entities and relationships of multi-relational data in low-dimensional vector spaces. Our objective is to propose a canonical model which is easy to train, contains a reduced number of parameters and can scale up to very large databases. Hence, we propose TransE, a method which models relationships by interpreting them as translations operating on the low-dimensional embeddings of the entities. Despite its simplicity, this assumption proves to be powerful since extensive experiments show that TransE significantly outperforms state-of-the-art methods in link prediction on two knowledge bases. Besides, it can be successfully trained on a large scale data set with 1M entities, 25k relationships and more than 17M training samples.
---------------------------------------------------------------
\cite{transh}
We deal with embedding a large scale knowledge graph composed of entities and relations into a continuous vector space.
TransE is a promising method proposed recently, which is
very efficient while achieving state-of-the-art predictive performance. We discuss some mapping properties of relations
which should be considered in embedding, such as reflexive, one-to-many, many-to-one, and many-to-many. We note
that TransE does not do well in dealing with these properties. Some complex models are capable of preserving these
mapping properties but sacrifice efficiency in the process. To
make a good trade-off between model capacity and efficiency,
in this paper we propose TransH which models a relation as a
hyperplane together with a translation operation on it. In this
way, we can well preserve the above mapping properties of
relations with almost the same model complexity of TransE.
Additionally, as a practical knowledge graph is often far from
completed, how to construct negative examples to reduce
false negative labels in training is very important. Utilizing
the one-to-many/many-to-one mapping property of a relation,
we propose a simple trick to reduce the possibility of false
negative labeling. We conduct extensive experiments on link
prediction, triplet classification and fact extraction on benchmark datasets like WordNet and Freebase. Experiments show
TransH delivers significant improvements over TransE on
predictive accuracy with comparable capability to scale up
---------------------------------------------------------------
\cite{katukuri2013semantic}
Embodiments of the present invention are generally related to systems, methods, computer readable media, and other means for extracting entities, determining the semantic relationships among the entities and generating knowledge. More particularly, some embodiments of the present invention are directed to generating a hypothesis and/or gaining knowledge by automatically extracting semantic relationships from electronic documents stored at remote databases, which are accessed over the Internet. Some embodiments of the present invention also include textual categorization and new approaches and algorithms for solving the problems of relationship extraction, computing semantic relationships and generating hypotheses.
---------------------------------------------------------------
\cite{CyberTwitter_Using_Twitter_to_generate_alerts_for_Cybersecurity_Threats_and_Vulnerabilities}
In order to secure vital personal and organizational system we require timely intelligence on cybersecurity threats and vulnerabilities. Intelligence about these threats is generally available in both overt and covert sources like the National Vulnerability Database, CERT alerts, blog posts, social media, and dark web resources. Intelligence updates about cybersecurity can be viewed as temporal events that a security analyst must keep up with so as to secure a computer system. We describe CyberTwitter, a system to discover and analyze cybersecurity intelligence on Twitter and serve as a OSINT (Open–source intelligence) source. We analyze real time information updates, in form of tweets, to extract intelligence about various possible threats. We use the Semantic Web RDF to represent the intelligence gathered and SWRL rules to reason over extracted intelligence to issue alerts for security analysts.
---------------------------------------------------------------
@article{JIA201853,
title = "A Practical Approach to Constructing a Knowledge Graph for Cybersecurity",
journal = "Engineering",
volume = "4",
number = "1",
pages = "53 - 60",
year = "2018",
note = "Cybersecurity",
issn = "2095-8099",
doi = "https://doi.org/10.1016/j.eng.2018.01.004",
url = "http://www.sciencedirect.com/science/article/pii/S2095809918301097",
author = "Yan Jia and Yulu Qi and Huaijun Shang and Rong Jiang and Aiping Li",
keywords = "Cybersecurity, Knowledge graph, Knowledge deduction",
abstract = "Cyberattack forms are complex and varied, and the detection and prediction of dynamic types of attack are always challenging tasks. Research on knowledge graphs is becoming increasingly mature in many fields. At present, it is very significant that certain scholars have combined the concept of the knowledge graph with cybersecurity in order to construct a cybersecurity knowledge base. This paper presents a cybersecurity knowledge base and deduction rules based on a quintuple model. Using machine learning, we extract entities and build ontology to obtain a cybersecurity knowledge base. New rules are then deduced by calculating formulas and using the path-ranking algorithm. The Stanford named entity recognizer (NER) is also used to train an extractor to extract useful information. Experimental results show that the Stanford NER provides many features and the useGazettes parameter may be used to train a recognizer in the cybersecurity domain in preparation for future work."
}
---------------------------------------------------------------
---------------------------------------------------------------
---------------------------------------------------------------
---------------------------------------------------------------
---------------------------------------------------------------
---------------------------------------------------------------
---------------------------------------------------------------




---------------------------------------------------------------
@article{DBLP:journals/corr/BridgesJIG13,
  author    = {Robert A. Bridges and
               Corinne L. Jones and
               Michael D. Iannacone and
               John R. Goodall},
  title     = {Automatic Labeling for Entity Extraction in Cyber Security},
  journal   = {CoRR},
  volume    = {abs/1308.4941},
  year      = {2013},
  url       = {http://arxiv.org/abs/1308.4941},
  archivePrefix = {arXiv},
  eprint    = {1308.4941},
  timestamp = {Mon, 13 Aug 2018 16:48:32 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/BridgesJIG13},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
Timely analysis of cyber-security information necessitates automated information extraction from unstructured text. While state-of-the-art extraction methods produce extremely accurate results, they require ample training data, which is generally unavailable for specialized applications, such as detecting security related entities; moreover, manual annotation of corpora is very costly and often not a viable solution. In response, we develop a very precise method to automatically label text from several data sources by leveraging related, domain-specific, structured data and provide public access to a corpus annotated with cyber-security entities. Next, we implement a Maximum Entropy Model trained with the average perceptron on a portion of our corpus (∼750,000 words) and achieve near perfect precision, recall, and accuracy, with training times under 17 seconds.
---------------------------------------------------------------
@inproceedings{Ritter:2015:WSE:2736277.2741083,
 author = {Ritter, Alan and Wright, Evan and Casey, William and Mitchell, Tom},
 title = {Weakly Supervised Extraction of Computer Security Events from Twitter},
 booktitle = {Proceedings of the 24th International Conference on World Wide Web},
 series = {WWW '15},
 year = {2015},
 isbn = {978-1-4503-3469-3},
 location = {Florence, Italy},
 pages = {896--905},
 numpages = {10},
 url = {https://doi.org/10.1145/2736277.2741083},
 doi = {10.1145/2736277.2741083},
 acmid = {2741083},
 publisher = {International World Wide Web Conferences Steering Committee},
 address = {Republic and Canton of Geneva, Switzerland},
 keywords = {information extraction, text mining},
} 
Twitter contains a wealth of timely information, however staying on top of breaking events requires that an information analyst constantly scan many sources, leading to information overload. For example, a user might wish to be made aware whenever an infectious disease outbreak takes place, when a new smartphone is announced or when a distributed Denial of Service (DoS) attack might affect an organization's network connectivity. There are many possible event categories an analyst may wish to track, making it impossible to anticipate all those of interest in advance. We therefore propose a weakly supervised approach, in which extractors for new categories of events are easy to define and train, by specifying a small number of seed examples. We cast seed-based event extraction as a learning problem where only positive and unlabeled data is available. Rather than assuming unlabeled instances are negative, as is common in previous work, we propose a learning objective which regularizes the label distribution towards a user-provided expectation. Our approach greatly outperforms heuristic negatives, used in most previous work, in experiments on real-world data. Significant performance gains are also demonstrated over two novel and competitive baselines: semi-supervised EM and one-class support-vector machines. We investigate three security-related events breaking on Twitter: DoS attacks, data breaches and account hijacking. A demonstration of security events extracted by our system is available at: http://kb1.cse.ohio-state.edu:8123/events/hacked
---------------------------------------------------------------
@inproceedings{Jones:2015:TRE:2746266.2746277,
 author = {Jones, Corinne L. and Bridges, Robert A. and Huffer, Kelly M. T. and Goodall, John R.},
 title = {Towards a Relation Extraction Framework for Cyber-Security Concepts},
 booktitle = {Proceedings of the 10th Annual Cyber and Information Security Research Conference},
 series = {CISR '15},
 year = {2015},
 isbn = {978-1-4503-3345-0},
 location = {Oak Ridge, TN, USA},
 pages = {11:1--11:4},
 articleno = {11},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/2746266.2746277},
 doi = {10.1145/2746266.2746277},
 acmid = {2746277},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {active learning, bootstrapping, cyber security, information extraction, natural language processing, relation extraction},
} 
In order to assist security analysts in obtaining information pertaining to their network, such as novel vulnerabilities, exploits, or patches, information retrieval methods tailored to the security domain are needed. As labeled text data is scarce and expensive, we follow developments in semi-supervised Natural Language Processing and implement a bootstrapping algorithm for extracting security entities and their relationships from text. The algorithm requires little input data, specifically, a few relations or patterns (heuristics for identifying relations), and incorporates an active learning component which queries the user on the most important decisions to prevent drifting from the desired relations. Preliminary testing on a small corpus shows promising results, obtaining precision of .82.

---------------------------------------------------------------
@MastersThesis{Information_Extraction_of_Security_related_entities_and_concepts_from_unstructured_text_,
	author = "Ravendar Lal",
	title = "{Information Extraction of Security related entities and concepts from unstructured text.}",
	month = "May",
	year = "2013",
	organization = "Ebiquity Lab",
	pages = "54",
	publisher = "University of Maryland Baltimore County",
}
Cyber Security has been a big concern especially in past one decade where it is witnessed that targets ranging from large number of internet users to government agencies are being attacked because of vulnerabilities present in the system. Even though these vulnerabilities are identified and published publicly but response has always been slow in covering up these vulnerabilities because there is no automatic mechanism to understand and process this unstructured text that is published on internet. Our system will be tackling this problem of processing unstructured text by identifying the security related terms including entities and concepts from various unstructured data sources. This information extraction task will help expediting the process of understanding and realizing the vulnerabilities and thus making systems secure at faster rate. This work will be describing a system that automatically extracts the terms from Cybersecurity blogs and security bulletins using Natural Language Processing (NLP) and text mining methods. Our NLP model is trained on manually annotated data using open-ended blogs and more structured text like company’s official security bulletins. This manually annotated data is unique of its kind since no such previous work has been done using this methodology and it can be a significant contribution for people working in this domain. Our named entity recognition model is trained on conditional random fields (CRFs) based Stanford NER. This automation system will be able to help administrators of organizations and governments to prioritize the task of beefing up their security and moreover track unofficial data sources like chat rooms and twitter for zero day attacks.
---------------------------------------------------------------
@inproceedings{Mulwad:2011:EIS:2052137.2052279,
 author = {Mulwad, Varish and Li, Wenjia and Joshi, Anupam and Finin, Tim and Viswanathan, Krishnamurthy},
 title = {Extracting Information About Security Vulnerabilities from Web Text},
 booktitle = {Proceedings of the 2011 IEEE/WIC/ACM International Conferences on Web Intelligence and Intelligent Agent Technology - Volume 03},
 series = {WI-IAT '11},
 year = {2011},
 isbn = {978-0-7695-4513-4},
 pages = {257--260},
 numpages = {4},
 url = {https://doi.org/10.1109/WI-IAT.2011.26},
 doi = {10.1109/WI-IAT.2011.26},
 acmid = {2052279},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {security, vulnerability, information extraction, entity linking},
} 
The Web is an important source of information about computer security threats, vulnerabilities and cyber attacks. We present initial work on developing a framework to detect and extract information about vulnerabilities and attacks from Web text. Our prototype system uses Wikitology, a general purpose knowledge base derived from Wikipedia, to extract concepts that describe specific vulnerabilities and attacks, map them to related concepts from DBpedia and generate machine understandable assertions. Such a framework will be useful in adding structure to already existing vulnerability descriptions as well as detecting new ones. We evaluate our approach against vulnerability descriptions from the National Vulnerability Database. Our results suggest that it can be useful in monitoring streams of text from social media or chat rooms to identify potential new attacks and vulnerabilities or to collect data on the spread and volume of existing ones.
---------------------------------------------------------------
@article{JIA201853,
title = "A Practical Approach to Constructing a Knowledge Graph for Cybersecurity",
journal = "Engineering",
volume = "4",
number = "1",
pages = "53 - 60",
year = "2018",
note = "Cybersecurity",
issn = "2095-8099",
doi = "https://doi.org/10.1016/j.eng.2018.01.004",
url = "http://www.sciencedirect.com/science/article/pii/S2095809918301097",
author = "Yan Jia and Yulu Qi and Huaijun Shang and Rong Jiang and Aiping Li",
keywords = "Cybersecurity, Knowledge graph, Knowledge deduction"
}
Cyberattack forms are complex and varied, and the detection and prediction of dynamic types of attack are always challenging tasks. Research on knowledge graphs is becoming increasingly mature in many fields. At present, it is very significant that certain scholars have combined the concept of the knowledge graph with cybersecurity in order to construct a cybersecurity knowledge base. This paper presents a cybersecurity knowledge base and deduction rules based on a quintuple model. Using machine learning, we extract entities and build ontology to obtain a cybersecurity knowledge base. New rules are then deduced by calculating formulas and using the path-ranking algorithm. The Stanford named entity recognizer (NER) is also used to train an extractor to extract useful information. Experimental results show that the Stanford NER provides many features and the useGazettes parameter may be used to train a recognizer in the cybersecurity domain in preparation for future work.
---------------------------------------------------------------
@INPROCEEDINGS{6693525, 
author={A. {Joshi} and R. {Lal} and T. {Finin} and A. {Joshi}}, 
booktitle={2013 IEEE Seventh International Conference on Semantic Computing}, 
title={Extracting Cybersecurity Related Linked Data from Text}, 
year={2013}, 
volume={}, 
number={}, 
pages={252-259}, 
keywords={data structures;information retrieval;Internet;meta data;ontologies (artificial intelligence);security of data;statistical analysis;text analysis;conditional random field;Web;cybersecurity linked data collection;DBpedia knowledge base;cybersecurity-related relations;cybersecurity-related concepts;cybersecurity-related entities;CRF-based system;National Vulnerability Database;vulnerability descriptions;RDF linked data representation;cybersecurity related linked data extraction;Ontologies;Data mining;Software;Resource description framework;Computer crime;cybeesecurity;linked data;information extraction;ontology}, 
doi={10.1109/ICSC.2013.50}, 
ISSN={}, 
month={Sep.},}
The Web is typically our first source of information about new software vulnerabilities, exploits and cyber-attacks. Information is found in semi-structured vulnerability databases as well as in text from security bulletins, news reports, cyber security blogs and Internet chat rooms. It can be useful to cyber security systems if there is a way to recognize and extract relevant information and represent it as easily shared and integrated semantic data. We describe such an automatic framework that generates and publishes a RDF linked data representation of cyber security concepts and vulnerability descriptions extracted from the National Vulnerability Database and from text sources. A CRF-based system is used to identify cybersecurity-relatedentities, concepts and relations in text, which are then represented using custom ontologies for the cyber security domain and also mapped to objects in the DBpedia knowledge base. The resulting cyber security linked data collection can be used for many purposes, including automating early vulnerability identification, mitigation and prevention efforts.

---------------------------------------------------------------

---------------------------------------------------------------

---------------------------------------------------------------

---------------------------------------------------------------

---------------------------------------------------------------

